Eclipsing White Dwarf Binaries in Gaia and the Zwicky Transient Facility

Gaia provided the largest-ever catalogue of white dwarf stars. We use this catalogue, along with the third public data release of the Zwicky Transient Facility (ZTF), to identify new eclipsing white dwarf binaries. Our method exploits light curve statistics and the Box Least Squares algorithm to detect periodic light curve variability. The search revealed 18 new binaries, of which 17 are eclipsing. We use the position in the Gaia H-R diagram to classify these binaries and find that the majority of these white dwarfs have main sequence companions. We identify one system as a candidate eclipsing white dwarf--brown dwarf binary and a further two as extremely low mass (ELM) white dwarf binaries. We also provide identification spectroscopy for 17 of our 18 binaries. Running our search method on mock light curves with real ZTF sampling, we estimate our efficiency of detecting objects with light curves similar to the ones of the newly discovered binaries. Many more binaries are to be found in the ZTF footprint as the data releases grow, so our survey is ongoing.

==> Response to referee/response.tex <==
We thank the referee for their comments and suggestions that will help to improve the clarity of this paper. We respond to the comments individually below and highlight substantial changes to the text in colour in the manuscript. 

A few days before we received the referee report, we were notified that we were awarded some observing time for spectroscopic confirmation of these binaries, scheduled for immediate observation. We carried out these observations and include the spectra in the paper. We apologise that this now makes for more substantial changes than might be expected, but it doesn't change the central message of the paper and we made sure to add the additional text in colour to highlight the changes. We have also added two additional co-authors who carried out the observations. The additional figures were added to the appendix, not to the main text. 




* My main issue is the presentation and discussion of the various sub-samples throughout the paper. The paper states (Sect. 4) that nine known eclipsing binaries plus 18 new systems are found by the automated period search. Please include a table with the nine known systems, and their basic properties. Do the overall properties of the nine known, and 18 new systems agree or differ?

Response: We added two tables to the appendix, to show the properties of the nine known binaries recovered by our search and the Burdge+2020 systems not recovered by our search. The tables have the same format as Table 1, which shows the properties of the new binaries. The overall properties are compared in Fig 4. 


* Section 6 states "We identified two binaries which potentially
contain ELM white dwarfs, one confirmed AM CVn star, one candidate white dwarf–brown dwarf binary, three cataclysmic variables, nine white dwarf–main sequence binaries, and two systems which likely have subdwarfs rather than white dwarfs as accretors." Does this refer to the 18 new systems? Could that information be presented also in tabular form? It is not trivial to sift through Sect. 5.3 to identify who is who.

Response: We added these classifications to Table 1, and also to the new tables in the appendix.



* Whenever you mention individual systems, or samples, be explicit. The caption of Fig. 4 reads "For reference, we have included eclipsing binaries listed in (Burdge et al. 2020a). Note that the two sources with negative skew are CVs with bright outbursts and that J1513+7037 is listed here..." I cannot decipher whether the two CVs are in Burdges sample, or among the newly identified systems.

Response: We have expanded the caption text to clarify which targets we are referring to.




* Section 4, "Apart from the negatively skewed source, all eclipsing binaries listed in Burdge et al. (2020a) lie above the cuts and would have therefore been included in our sample provided that they were contained in the white dwarf catalogue of Gentile Fusillo" Were they? How many of Burdge's systems are in the GF catalogue, how many made it through the other data quality cuts?

Response: We have added the details of these sources to the text



* In Section 5.1, currently named "Completeness", "also detected a number of known or recently-identified systems", "However, it is also notable that some known systems were not detected in this initial search. This is likely due to the target selection method we chose, which requires the target to be included in the Gaia white dwarf catalogue.", "it is also possible that some systems were lost in the initial cuts".
=> All these vague terms need to be quantified. How many are "a
number", "some" and "likely ... target selection" - you defined the target selection, and have all information at hand to quantify "likely" and "possible".

Response: Those sentences were meant as an 'introduction' to the discussion following them, where the details are quantified. We re-wrote that paragraph to clarify what we mean.  


* As a test, the authors compared the binaries they found "to the known eclipsing binaries in the International Variable Star Index database, VSX" It is not clear what that means: VSX will contain *many* eclipsing binaries, most of which don't contain a white dwarf component. I believe that some cross-match between VSX and the white dwarf catalogue of Gentile Fusillo was done to thin out the VSX eclipsing binary list, however, that is not clear.
But, another important question is: how complete is VSX on eclipsing white dwarf binaries? Without the answer to that question, using VSX to test the completeness of their search is bound to lead to unreliable results. 

If the authors want to carry out an assessment of their
completeness, I would urge them to identify from the literature
known eclipsing white dwarf binaries, e.g.
https://ui.adsabs.harvard.edu/abs/2015MNRAS.448..601B
https://ui.adsabs.harvard.edu/abs/2010ApJ...716L.146S
https://ui.adsabs.harvard.edu/abs/2016MNRAS.458..845H
https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.4473P
https://ui.adsabs.harvard.edu/abs/2017ApJ...847...10B
https://ui.adsabs.harvard.edu/abs/2011ApJ...737L..16V
then work out how many of those fall into their target selection and further data quality cuts, and finally work out how many of them are recovered by their search (which should hence be among the nine known eclipsing systems).
All of this is laborious and tedious, and the authors may consider to drop this sub-section altogether.



Response: We believe that an attempt at a completeness analysis (however hard it is) is a very important part of any systematic search for a particular objects, and so strongly disagree that this section should be dropped. 
The difficulty, as we stated in the paper and was pointed out by the referee as well, is that we don't exactly know the completeness of VSX. However, VSX is doing an amazing job of maintaining a record of published photometrically variable stars (including eclipsing binaries) and every white dwarf binary we were able to find in the literature was already included in VSX. This includes all the eclipsing binaries in all the papers listed by the referee. We therefore believe that comparing to VSX gives a good comparison to the known eclipsing white dwarfs. Of course, we don't know what we don't know, and that is the point of the simulations we've done: to show how the number of observations (in ZTF) affects our ability to recover eclipsing white dwarfs and show where our search might be incomplete. 

We have updated the text with a few more details for clarity, but the original version already included a detailed paragraph explaining the details of our WD catalogue/VSX cross-match and the subsequent cuts. 





* Sect. 5.2, note that a similar analysis was carried out by Parsons et al. https://ui.adsabs.harvard.edu/abs/2013MNRAS.429..256P, and it would be useful to compare the results obtained here with that study.

Response: Any completeness analysis is specific to the survey properties and the method used to uncover the targets of interest. The Parsons et al 2013 study is excellent, but it is very different to what we do here. It focused specifically on WDMS binaries, with periods appropriate to those systems. Their longest period system has P=1.93d, which is much longer than our maximum 2.4hr searched. Of the 30 eclipsers they identify, only 3 fall into the period range we searched. It is also based on a survey (CRTS) with a very different cadence to ZTF, and for which they had access to the survey imaging data. The results from the two studies cannot therefore be compared directly.


* The introduction focuses largely on double-white dwarfs and AM CVn systems, however, the identified systems are mainly white dwarfs with low-mass stellar companions. These two aspects should be aligned better.

Response: The introduction reflects our initial motivation for this project and gives credit to the ZTF team for their discoveries. We have added an additional paragraph to explain the main difference in our search criteria and how that might affect the type of binaries we find, as well as a paragraph about WDMS binaries.


* Sect. 3.1, "Hence, a significant detection of a double degenerate system becomes less likely at longer periods." again, the focus is set on double-degenerates, of which few are found.

Response: This comment refers more generally to eclipsing binaries, not just double degenerates, so we have updated the text to reflect this.


* Sect. 4 includes some discussion of the kinematic properties,
concluding that "(most) of our binaries are denizens of the Galactic thick disc instead" - is that surprising? What are the implications? Are these predominantly old systems?

Given the variety of binaries detected here, we thought it important to check their distribution within the Galaxy. While the result is not surprising, it shows that we need a bigger volume to pick up rare systems, which implies going further out into the thick disc. We also note that while ZTF observes in the plane, it is, on average, a high $b$ survey, which means we are more likely to detect objects from the thick disc.



* Table 1: what are the uncertainties on P and T_0? \omega is slightly unusual as choice for parallax?

Response: The uncertainties were originally included in the caption of Table 1 but it seems to have disappeared in a recent edit. Thanks for noticing that, we have re-added it now.

\omega is a common way of referring to parallax, and, importantly, the way adopted for the Gaia data releases. Given that we rely on the Gaia data in this work, we follow the same convention. 


* The quality of the figures could be improved by using a single
font. The current presentation of the light curves (Fig. 7, 9, 10, 12-14) takes up a lot of space with relatively low information density => move to an appendix?

We changed the figures to all use the same (non-math, Sans Serif) font. 
We believe that it is important to show the light curves that the binary identification is based on, so that the readers can be convinced of their quality and the reliability of the detection. The figures also show our fits to the eclipses and the results of the simulations (to test the importance of the number of points in the light curve), so we prefer to leave them in as part of the main paper. 



==> Response to referee/response2.tex <==
We again thank the referee for their comments, especially point (ii) which was a mistake on our part. These binaries are indeed detached systems with a subdwarf primary, the word accretor is out of place here. We've corrected that now. 

On point (i) we agree with the referee that VSX cannot be considered "ground truth". We've added a few sentences explaining that the specific investigation we've done refers only to the internal completeness, i.e. how thoroughly we searched the sample, given our stated criteria. The external completeness, which we think is what the referee refers to, is not possible to estimate without some "ground truth" catalogue or model. We've added comments about that to Section 5.1. 

As before, all changes are highlighted in colour for easy reference. 
